Projection-free Graph-based Classifier Learning using Gershgorin Disc Perfect Alignment

In semi-supervised graph-based binary classifier learning, a subset of known labels $\hat{x}_i$ are used to infer unknown labels, assuming that the label signal $\mathbf{x}$ is smooth with respect to a similarity graph specified by a Laplacian matrix. When restricting labels $x_i$ to binary values, the problem is NP-hard. While a conventional semi-definite programming relaxation (SDR) can be solved in polynomial time using, for example, the alternating direction method of multipliers (ADMM), the complexity of projecting a candidate matrix $\mathbf{M}$ onto the positive semi-definite (PSD) cone ($\mathbf{M} \succeq 0$) per iteration remains high. In this paper, leveraging a recent linear algebraic theory called Gershgorin disc perfect alignment (GDPA), we propose a fast projection-free method by solving a sequence of linear programs (LP) instead. Specifically, we first recast the SDR to its dual, where a feasible solution $\mathbf{H} \succeq 0$ is interpreted as a Laplacian matrix corresponding to a balanced signed graph minus the last node. To achieve graph balance, we split the last node into two, each retains the original positive / negative edges, resulting in a new Laplacian $\bar{\mathbf{H}}$. We repose the SDR dual for solution $\bar{\mathbf{H}}$, then replace the PSD cone constraint $\bar{\mathbf{H}} \succeq 0$ with linear constraints derived from GDPA -- sufficient conditions to ensure $\bar{\mathbf{H}}$ is PSD -- so that the optimization becomes an LP per iteration. Finally, we extract predicted labels from converged solution $\bar{\mathbf{H}}$. Experiments show that our algorithm enjoyed a $28\times$ speedup over the next fastest scheme while achieving comparable label prediction performance.

==> reviewer_4zJS.tex <==
\textbf{Overall Comment}:
\textit{The authors propose an efficient algorithm for a semi-supervised classification problem, applicable for graphs (i.e., each node receives a binary label). Specifically, the problem assumes that we have available a weighted undirectional graph where a subset of the nodes are labeled (as 1, or -1). The goal is to estimate the labels of the remaining nodes, while respecting the graph structure imposed by the available edge weights. For this, the authors consider a well-known formulation, which requires solving a computationally challenging non-convex (discrete) minimization problem. In order to make it computationally tractable, they resort to a common SDP relaxation. Noting that such relaxation can be computationally demanding, due to the need to perform a projection onto the positive semi-definite code, the authors leverage a recent result that provides simple tight bounds on the minimum eigenvalue of special matrices (Laplacian matrices of balanced graphs). In order to employ this result, they consider the dual of the SDP relaxed problem, and further modify this dual to reach a formulation for which the mentioned bounds apply. Employing these bounds allow them to devise an algorithm that requires a minimum eigenvector computation, followed by solving a linear program. They demonstrate numerically that this scheme compares favorably against existing approaches.}

\textit{The paper makes use of a recent result (Gershgorin disc perfect alignment -- GDPA) to modify a matrix (through a similarity transformation) so as to obtain tight bounds (via Gershgorin discs) on the minimum eigenvalue of the matrix. In order to apply the result, the authors go through multiple stages of transforming the problem of interest, namely semi-supervised graph classifier learning. Overall, I think the paper is potentially interesting in terms of demonstrating how GDPA can be employed to tackle a common formulation of this specific problem. However, I also found the paper to be terse, unclear at times.}

\vspace{0.4cm}
\noindent
\textbf{Overall Response}: 
We thank the reviewer for a very thorough reading of our submission.
We note that all of the reviewer's comments are concerns about presentation clarity, which can be easily addressed with a careful revision.
There were no technical criticisms of the proposed optimization strategy.
We note also that the reviewer's comments on unclear writeup contradict comments by reviewer EGbx, who stated that our paper is "easy to follow" and our contribution "is clear". 

% %----------------------------------------------------- Q1
\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
\textit{in various places the expression "sans the last node" appears, I'd suggest replacing "sans" with "without"?}

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
We will be happy to replace the preposition "sans" with "without" in the final version of the paper, though it is stated in the Merriam-Webster dictionary that the two words are equivalent:
\begin{quote}
https://www.merriam-webster.com/dictionary/sans
\end{quote}
% We thank the reviewer for this comment, and we apologize for the imprecise specification in our previous Algorithm 1.
% In the revised manuscript, we included a new metric matrix initialization procedure in Section 4.2.1, which outputs a generalized graph Laplacian matrix $\M^0$ corresponding to a balanced signed \textit{tree graph} $\cG$ and corresponding blue and red node sets $\cN_b$ and $\cN_r$. 
% These are the inputs to the pseudo-code of Algorithm 1. 
% Note also that we have rewritten the pseudo-code of Algorithm 1 in the revised manuscript for improved clarity.

% %----------------------------------------------------- Q2
\vspace{1.0cm}
\noindent
\textbf{Comment 2}: 
\textit{Introduction : It would be useful to introduce the notion of a "balanced graph" with a proper definition. In particular, you can mention that a graph with positive edge weights is balanced.}

\vspace{0.4cm}
\noindent
\textbf{Response 2}: 
The definition of a balanced graph is provided in line 109 of page 3 (Section 3.2) of the submission: "A balanced graph is a graph with no cycle of odd number of negative edges". 

As the reviewer has pointed out, a straightforward corollary of this definition is that a positive graph is always balanced.
We will include this detail in the final version of the paper to facilitate understanding.
% %\red{Clarify pseudo-code.}
% We apologize for the unclear specification in previous Algorithm 1.
% In the rewritten Algorithm 1 in the revised manuscript, we have removed wordings ``Do 3--8" and replaced them with while loops for improved clarity.

% %----------------------------------------------------- Q3
\vspace{1.0cm}
\noindent
\textbf{Comment 3}: 
\textit{If the graph doesn't have self loops, typically the first eigenvector of Laplacian matrices for graphs with positive weights is all ones (with zero eigenvalue) -- for readers not expecting self-loops, it might be good to mention the existence of self-loops.}

\vspace{0.4cm}
\noindent
\textbf{Response 3}: 
In the formal definition of a graph in Section 3.1, it is stated clearly that each graph node may have a self-loop: "A node $i$ may have self-loop of weights $u_i \in \mathbb{R}$" (line 98 in page 3).
% We thank the reviewer for this comment. 
% In the revised manuscript, we have added experimental comparisons with the conference version of this work that considered only graph metric matrices corresponding to positive graphs only. 
% As shown in Tables\;3 and 4 of the revised manuscript, we can see that considering graph metric matrices of more general balanced signed graphs (SGML) outperformed positive graphs (PGML) for almost all objectives $Q(\M)$ and datasets. 
% This demonstrates that it is worth the extra effort to consider the more general case of signed graphs as proposed in this paper. 

% %\blue{Cheng: We added our previous work that is also based on GDPA but within a positive graph metric space, namely, PGML \cite{yang20}. In our revised manuscript, we added the results of PGML on the objective values in Tables 3 and 4, and the classification accuracy in Tables 6 and 7. For objective values in Tables 3 and 4, our previous PGML achieved larger (for MCML, LSML, LMNN and GLR minimization problems) and smaller (for DEML maximization problem) averaged objective values over a high-complexity optimal scheme PD-cone, \textit{i.e.}, the further objective values compared to PD-cone, compared to our proposed SGML optimization scheme. As shown in the last column of Tables 3 and 4, our proposed SGML performed generally better than our previous work PGML \cite{yang20} that has generally much more restrictive metric space and has sub-optimal solutions for MCML, DEML, LSML, LMNN and GLR objectives. For classification accuracy, our previous PGML achieved comparable classification accuracy against PD-cone, and HBNB and our proposed SGML given the fact that PGML has much less time-complexity compared to the optimal scheme PD-cone. }

% %----------------------------------------------------- Q4
\vspace{1.0cm}
\noindent
\textbf{Comment 4}: 
\textit{line 53 : The sentence starting with "This means that transformed...". Is the equality $\lambda^- = \lambda$ (i.e., tight bound) obvious? Again, for readers not familiar with GDPA development, it might be good to mention this is a consequence of the GDPA development, because the bound is not tight for regular Gershgorin discs, as you state elsewhere.}

\vspace{0.4cm}
\noindent
\textbf{Response 4}: 
We note that the preceding sentence to line 53 succinctly summarized the main conclusion of GDPA in [11]: 
\begin{quote}
Specifically, GDPA states that given a graph Laplacian matrix $\L$ corresponding to a balanced signed graph $\cG$ [12], one can perform a similarity
transform, $\tilde{\L} = \S \L \S^{-1}$ where $\S = \text{diag}(v_1, \ldots, v_N)$ and $\v$ is the first eigenvector of $\L$, such that the Gershgorin disc left-ends of $\tilde{\L}$ are exactly aligned at $\lambda_{\min}(\L) = \lambda_{\min}(\L)$.
\end{quote}
Given the definition of GCT lower bound $\lambda^-_{\min}(\M) \triangleq \min_i c_i(\M) - r_i(\M)$ in (2), it does mean that $\lambda^- = \lambda$ (\ie, tightest possible) in this case.
We note further that this special similarity transform due to GDPA to align Gershgorin disc left-ends at the smallest eigenvalue $\lambda_{\min}(\M)$ is graphically illustrated in Fig.\;1.

% %----------------------------------------------------- Q5
\vspace{1.0cm}
\noindent
\textbf{Comment 5}: 
\textit{Section 3.1 : It might be good to introduce "balanced graphs" properly here, since it is a key concept for GDPA (and generalizes graphs with positive edge weights).}

\vspace{0.4cm}
\noindent
\textbf{Response 5}: 
The definition of a balanced graph is clearly stated in Section 3.2 (line 109 of page 3): "A balanced graph is a graph with no cycle of odd number of negative edges."
Instead of this hard-to-use original definition, we also further explained that "By Cartwright-Harary Theorem (CHT) [12], a graph is balanced iff nodes can be colored into blue and red, such that each positive (negative) edge connects nodes of the same (different) colors."
While one may dispute the most appropriate locations of these definitions (Section 3.1 versus Section 3.2), it is clear that these definitions were included in the original submission.
We will be happy to move the definitions of a balanced graph from Section 3.2 to Section 3.1 in the final version of the paper, as recommended by the reviewer. 

% %----------------------------------------------------- Q6
\vspace{1.0cm}
\noindent
\textbf{Comment 6}: 
\textit{Section 3.2 : I recommend including a clear statement of GDPA (possibly along with necessary definitions), since the purpose of the paper is to apply it to a particular problem. Any additional discussion, insight is welcome.}

\vspace{0.4cm}
\noindent
\textbf{Response 6}: 
The key idea of GDPA---the alignment of Gershgorin disc left-ends at smallest eigenvalue $\lambda_{\min}(\M)$ of a generalized graph Laplacian matrix $\M$ corresponding to a balanced signed graph via a similarity transform $\S \M \S^{-1}$---is clearly described in the Introduction and intuitively illustrated in Fig.\;1. 
A more rigorous mathematical definition is already provided starting at line 111 of page 3 (Section 3.2) of the submission. 
% \dandel{With due respect to the reviewer, we do not understand what the reviewer is requesting that is not already included in the paper. }
% \dancomment{We will keep in mind the importance of the connection with GDPA in our subsequent revisions.}
We will keep in mind the importance of the connection with GDPA in our subsequent revisions.

% %----------------------------------------------------- Q7
\vspace{1.0cm}
\noindent
\textbf{Comment 7}: 
\textit{Paragraph starting at line 148 : I think this discussion is important, but currently, it's really abrupt. Specifically, if you could spare a few more words on how in general M could/should be interpreted as an adjacency matrix.}

\vspace{0.4cm}
\noindent
\textbf{Response 7}: 
This discussion here is indeed important and motivates the study of the SDP dual.
However, we are puzzled by this reviewer comment, because the interpretation of $\M$ as an adjacency matrix of a signed graph is already illustrated graphically in Fig.\;2(b) as a 4-node graph.
For example, reading the first row $[1 ~-1 ~1 ~1]$ of matrix $\M$ in (9), we connect node pairs $(1,2)$, $(1,3)$ and $(1,4)$ with weights $w_{1,2} = -1$, $w_{1,3} = 1$ and $w_{1,4} = 1$, respectively. 
(As mentioned in the figure caption, self-loops $u_i$'s---which do not affect graph balance---are omitted for simplicity.)
As illustrated, this 4-node signed graph is a \textit{balanced} graph: nodes $1$, $3$ and $4$ are colored blue while node $2$ is colored red, so that positive (negative) edges always connect nodes of the same (different) colors.
This shows that the solution to the original SDP primal problem exhibits the desired graph balance property, albeit in exactly the wrong signs, since GDPA requires a \textit{Laplacian} matrix corresponding to a balanced signed graph, which has the exact opposite signs as the adjacency matrix in the off-diagonal terms.
This motivates the study of the SDP dual instead.

In the final version of the paper, to further facilitate understanding, we will elaborate on the construction of the 4-node graph in Fig.\;2(b) from matrix $\M$ as described above. 

% %----------------------------------------------------- Q8
\vspace{1.0cm}
\noindent
\textbf{Comment 8}: 
\textit{Also, in and of itself, this doesn't motivate the consideration of the dual, is that right? The form of H in the dual resembles a Laplacian, because it contains L, which appears in the cost function of the primal problem.}

\vspace{0.4cm}
\noindent
\textbf{Response 8}: 
From response 7 above, we see that the solution to the SDP primal in (8) is an \textit{adjacency} matrix corresponding to a balanced signed graph, which makes it difficult to apply GDPA linearization that demands a \textit{graph Laplacian} matrix with opposite signs in the off-diagonal terms to the adjacency matrix.
Thus, leveraging on SDP duality theory \cite{gartner12}, we investigate the corresponding SDP dual (12) instead, which turns out has a solution that is a graph Laplacian matrix corresponding to a balanced signed graph (minus the last node), and hence amenable to GDPA linearization. 

% %----------------------------------------------------- Q9
\vspace{1.0cm}
\noindent
\textbf{Comment 9}: 
\textit{line 158 instead of "We derive", I would suggest using "We state", since there's no derivation in this section. Is (12) obtained from the Lagrangian dual of (8)? If so, I suggest to mention this explicitly. If there are additional hoops one needs to jump through, it would be good to note that as well.}

\vspace{0.4cm}
\noindent
\textbf{Response 9}: 
The reviewer is correct in claiming that it is more appropriate to use "We state" instead of "We derive" in line 158, since the derivation of the SDP dual was obmitted in the main manuscript due to lack of space. 
We will make this correction in the final version of this paper.

The mapping from the SDP primal to the corresponding SDP dual is a straightforward (albeit mundane) one following procedure in SDP duality theory described in optimization textbooks such as \cite{gartner12}.
There are no "additional hoops one needs to jump through". 
We will clarify this SDP duality mapping in the final version of this paper.


% %----------------------------------------------------- Q10
\vspace{1.0cm}
\noindent
\textbf{Comment 10}: 
\textit{line 164, sentence starting with "Because the objective is a minimization, when $b_i < 0, ... z_i \geq 0$" : I'd agree with this statement if the problem (12) were unconstrained. But $z_i$'s also appear in the constraints -- is the statement still obvious?}

\vspace{0.4cm}
\noindent
\textbf{Response 10}: 
We agree with the reviewer's comment that this statement is not obvious and deserves a clearer explanation in the final version of this paper. 
The statement is true because each $\B_i$, defined in (10), contains only off-diagonal terms that would strictly increase the radii of Gershgorin discs $i$ and $N+1$ of matrix $\H$ in (12), regardless of the sign of $z_i$, thus making the requirement $\H \succeq 0$ more difficult.
Thus, if $b_i < 0$, then $z_i < 0$ does not make sense, since it would increase the minimization objective \textit{and} worsen the PSDness of matrix $\H$ in the PSD cone constraint $\H \succeq 0$.

% %----------------------------------------------------- Q11
\vspace{1.0cm}
\noindent
\textbf{Comment 11}: 
\textit{line 171 vs eqn (12) : According to eqn (12), shouldn't we have $L_y = \mathrm{diag}(y_i) - L$, as opposed to $\mathrm{diag}(y_i) + L$, as written in line 171?}

\vspace{0.4cm}
\noindent
\textbf{Response 11}:
The definition of $\cL_y = \text{diag}(y_i) + \L$ is correct. 
However, there was a minor mistake in equation (12) of the submitted manuscript, where instead of $-\L$ in the definition of $\H$, it should be $\left[\begin{array}{cc}
\L & \0_N \\
\0_N^{\top} & 0
\end{array}\right]$.
We will correct this error in the final version of the paper. 

%\blue{Cheng: We apologize for the confusion. $\cL_y=\mathrm{diag}(y_i) + \L$ in line 171 is correct, but there was an error in the last term $-\L$ of eqn (12) where it should be $+\left[\begin{array}{cc}
%\L & \0_N \\
%\0_N^{\top} & 0
%\end{array}\right] $. 
%We also apologize for a similar error in the last term $-\L$ of eqn(20) where it should be $+\left[\begin{array}{cc}
%\L & \0_{N+2} \\
%\0_{N+2}^{\top} & 0_{2\times2}
%\end{array}\right]$. }

% %----------------------------------------------------- Q12
\vspace{1.0cm}
\noindent
\textbf{Comment 12}: 
\textit{eqn (21) : these work for any $s_i$, don't they (since we're performing a similarity transformation and resorting to bounds obtained from Gershgorin discs)? Even though arbitrary Gershgorin disc bounds may not be tight, they wouldn't lead to solutions that violate any constraints. By including $v_i$'s as you define here, you essentially work with the "best possible" before attempting to solve the LP. If you agree with this comment, I'd suggest including something in this direction in the text as well.}

\vspace{0.4cm}
\noindent
\textbf{Response 12}: 
The reviewer is correct that \textit{any} similarity transform $\S \bar{\H} \S^{-1}$ such that $\lambda^-_{\min}(\S \bar{\H} \S^{-1}) \geq 0$ would ensure that matrix $\bar{\H}$ is PSD.
In other words, $\lambda^-_{\min}(\S \bar{\H} \S^{-1}) \geq 0$ for any $\S$ is a sufficient (but not necessary) condition for $\M \succeq 0$. 
However, the only way to obtain the \textit{tightest possible} linear constraints, \ie, $\lambda^-_{\min}(\S \bar{\H} \S^{-1}) = \lambda_{\min}(\S \bar{\H} \S^{-1}) =  \lambda_{\min}(\bar{\H})$, is to invoke GDPA theory: i) compute the first eigenvector $\v$ of generalized graph Laplacian $\bar{\H}$ for a balanced signed graph, and ii) compute $\S = \text{diag}(v_1, \ldots, v_N)$. 
Using any other invertible matrix $\S$ to impose linear constraints $\lambda^-_{\min}(\S \bar{\H} \S^{-1}) \geq 0$ would mean an unnecessary restriction in the search space for $\bar{\H}$, resulting in sub-optimal optimization performance.
We will clarify this point in the final version of the paper. 

==> reviewer_EGbx.tex <==
\textbf{Overall Comment}:
\textit{This paper proposes a method based on the Gershgorin Disc Perfect Alignment (GDPA) to efficiently solve a binary semi-supervised learning problem over graphs. In short, the semi-supervised learning problem can be naturally relaxed to an SDP problem through the well-established lifting operation. The authors claim that projecting to the PSD cone can be time consuming and, instead, propose an approach to ensure that the smallest eigenvalue is non-negative (thus, the matrix being PSD) based on the GDPA, which can be encoded as a series of linear constraints. This reformulation is actually achievable in the dual of the original SDP since the tightness of the GDPA approach requires certain assumptions that are not satisfied in the primal.}

\textit{The paper is easy to follow. The contribution is not huge but it is clear. The use of the GDPA technique could go beyond the problem considered here and this paper can serve as an example of its implementation. In that sense, the value of the contribution can go beyond the specific problem of binary supervised learning on graphs. My main criticism has to do with the comparisons with other methods in Section 6. The authors consider comparisons mainly with SDP methods (except for BCR), thus showing the computational gain with respect to these SDP baselines. However, there is no comparison with simpler non-convex methods beyond BCR and, more importantly, with very simple relaxations like relaxing the binary constraint to a box constraint [-1, 1] and minimizing the quadratic Laplacian loss. A minimization like that one can probably be implemented very fast, but presumably has worse performance? There is no such comparison in the paper.}

\vspace{0.4cm}
\noindent
\textbf{Overall Response}: 
We thank the reviewer for the overall positive comment. 
We first note that SDP relaxation to the general NP-hard quadratically constrained quadratic programs (QCQP), which include our semi-supervised graph classifier learning problem as a special case, is well accepted in the convex optimization and signal processing communities, given its proven approximation bounds for many practical cases of interest (see Table I and II in \cite{5447068}). 
%\cite{5447068} \blue{Cheng: not sure if we include the following reference \cite{equivalent_box_sdp} (see Table 1 in \cite{equivalent_box_sdp}) which shows that the box-constraint relaxation has the same bound as the semidefinite relaxation. Does this mean that the box-constraint relaxation can ideally achieve the same accuracy as the semidefinite relaxation?}. 
In contrast, to the best of our knowledge, ad-hoc relaxation of the binary constraint to box constraint does not have bounded approximation performance guarantees for QCQP. 
Given the acceptance of SDP relaxation in the optimization community, our goal is simply to reduce the execution time of SDP relaxation via GDPA linearization, which we have demonstrated thoroughly in our experiments. 

Nonetheless, as suggested by the reviewer, we have implemented the box constraint based method with a CVX solver (denoted as "BOX").
We found that, using the same 17 datasets in the results section, our GDPA linearization proposal is on average 0.48\% (for min-max data re-scaling) and 1.46\% (for standardization data re-scaling) smaller than BOX in classification error rates, 
and on average 59$\times$ faster than BOX in runtime. 
We will include this new comparison result in the final version of this paper.
% \red{I don't think you should present fine-grained results here. just summarize your results and say that in your experiments, you found that our proposal is better than a box constraint scheme by classification error by $X\%$ on average, and faster by $X\times$ when using GLR-box for optimization routine (CVX).} 
% In particular, we implemented the box constraint based method (suggested by the reviewer) with a CVX solver (denoted as "GLR-box (CVX)") and conducted experiments using the same 17 datasets in the experimentation section.
% The averaged classification error rates and runtime are shown below:

% 1. error rates (\%) and runtime (ms) for min-max data re-scaling:\\
% SeDuMi, MOSEK, CDCS(8), BCR, SDcut, CDCS(20), GDPA, GLR-box (CVX)\\
% ---classification error rate ($\%$): $32.36, 32.59, 32.40, 28.78, 28.78, 29.26, 29.13, 29.61$\\
% ---runtime (ms): $1475.41, 800.46, 2183.70, 516.79, 361.39, 477.08, 5.92, 296.82$\\

% % |         |  SeDuMi |  MOSEK | CDCS (8) |   BCR  |  SDcut | CDCS (20)  |  GDPA | GLR-box (CVX) |
% % |:------------------------------:|:-------:|:------:|:--------:|:------:|:------:|:----------:|:-----:|:-------------:|
% % | classification error rate (\%) |  32.36  |  32.59 |   32.40  |  28.78 |  28.78 |    29.26   | 29.13 |     29.61     |
% % |          runtime (ms)          | 1475.41 | 800.46 |  2183.70 | 516.79 | 361.39 |   477.08   |  5.92 |     296.82    |

% 2. error rates (\%) and runtime (ms) for standardization data re-scaling:\\
% SeDuMi, MOSEK, CDCS(8), BCR, SDcut, CDCS(20), GDPA, GLR-box (CVX)\\
% ---classification error rate ($\%$): $32.81, 32.83, 33.22, 26.47, 27.13, 27.18, 27.14, 28.50$\\
% ---runtime (ms): $1892.32, 938.84, 3009.23, 53.17, 606.49, 499.72, 5.62, 303.12$

% % |    |  SeDuMi |  MOSEK | CDCS (8) |  BCR  |  SDcut | CDCS (20)  |  GDPA | GLR-box (CVX) |
% % |:-------------------------------:|:-------:|:------:|:--------:|:-----:|:------:|:----------:|:-----:|:-------------:|
% % |  classification error rate (\%) |  32.81  |  32.83 |   33.22  | 26.47 |  27.13 |    27.18   | 27.14 |     28.50     |
% % |           runtime (ms)          | 1892.32 | 938.84 |  3009.23 | 53.17 | 606.49 |   499.72   |  5.62 |     303.12    |

% The above results show that, our proposed GDPA is $0.48\%$ ($29.13\%$ vs $29.61\%$) and $1.46\%$ ($27.14\%$ vs $28.50\%$) better than GLR-box (CVX) in the classification error rates, respectively.
% The proposed GDPA is also about $59\times$ ($5.92$ms vs $296.82$ms, and $5.62$ms vs $303.12$ms) faster than GLR-box (CVX).

% %----------------------------------------------------- Q1
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 1}: 
% \textit{You should provide explicit bounds on the time complexity of full eigen-solvers $\mathcal{O}(n^3)$ versus your approach, i.e., solving a sequence of LPs. What is the time complexity of your proposed approach?}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 1}: 
% We thank the reviewer for this comment, and we apologize for the imprecise specification in our previous Algorithm 1.
% In the revised manuscript, we included a new metric matrix initialization procedure in Section 4.2.1, which outputs a generalized graph Laplacian matrix $\M^0$ corresponding to a balanced signed \textit{tree graph} $\cG$ and corresponding blue and red node sets $\cN_b$ and $\cN_r$. 
% These are the inputs to the pseudo-code of Algorithm 1. 
% Note also that we have rewritten the pseudo-code of Algorithm 1 in the revised manuscript for improved clarity.

% %----------------------------------------------------- Q2
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 2}: 
% \textit{What is the time complexity of computing the eigenvector corresponding to the smallest eigenvalue? Can you bound $b$ in L116? As far as I know, computing the smallest eigenvalue/vector is as hard as computing the full eigen-decomposition. Please clarify and be precise in your statements otherwise.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 2}: 
% $b$ in L116 was set to 200 as mentioned in L246 in Section 6.1.
% %\red{Clarify pseudo-code.}
% We apologize for the unclear specification in previous Algorithm 1.
% In the rewritten Algorithm 1 in the revised manuscript, we have removed wordings ``Do 3--8" and replaced them with while loops for improved clarity.

% %----------------------------------------------------- Q3
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 3}: 
% \textit{Section 5.1. You need to provide a bound on the number of iteration of your GDPA linearization process. How many steps are required to achieve an approximate solution? Please elaborate if there is any bound on the rate of convergence.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 3}: 
% We thank the reviewer for this comment. 
% In the revised manuscript, we have added experimental comparisons with the conference version of this work that considered only graph metric matrices corresponding to positive graphs only. 
% As shown in Tables\;3 and 4 of the revised manuscript, we can see that considering graph metric matrices of more general balanced signed graphs (SGML) outperformed positive graphs (PGML) for almost all objectives $Q(\M)$ and datasets. 
% This demonstrates that it is worth the extra effort to consider the more general case of signed graphs as proposed in this paper. 

% %\blue{Cheng: We added our previous work that is also based on GDPA but within a positive graph metric space, namely, PGML \cite{yang20}. In our revised manuscript, we added the results of PGML on the objective values in Tables 3 and 4, and the classification accuracy in Tables 6 and 7. For objective values in Tables 3 and 4, our previous PGML achieved larger (for MCML, LSML, LMNN and GLR minimization problems) and smaller (for DEML maximization problem) averaged objective values over a high-complexity optimal scheme PD-cone, \textit{i.e.}, the further objective values compared to PD-cone, compared to our proposed SGML optimization scheme. As shown in the last column of Tables 3 and 4, our proposed SGML performed generally better than our previous work PGML \cite{yang20} that has generally much more restrictive metric space and has sub-optimal solutions for MCML, DEML, LSML, LMNN and GLR objectives. For classification accuracy, our previous PGML achieved comparable classification accuracy against PD-cone, and HBNB and our proposed SGML given the fact that PGML has much less time-complexity compared to the optimal scheme PD-cone. }

% %----------------------------------------------------- Q4
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 4}: 
% \textit{The abstract is very hard to follow. I would highly recommend that the authors make an attempt to rewrite it. For example, the problem studied is not clear and in L4 is stated that it is NP-hard. Complexity is high (L8) can be more precise. Last but not least, please do not state in the abstract step-by-step how you approach the problem but only state the key insights, i.e., use of GDPA theory and LPs. Removing the part, "Specifically,... per iteration" would remove a lot of unnecessary details.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 4}: 

% %----------------------------------------------------- Q5
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 5}: 
% \textit{Please define the optimization problem in introduction more precisely. For example, what is optimized exactly? Please do not assume the reader is familiar with the problem under study.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 5}: 

==> reviewer_WMZZ.tex <==
\textbf{Overall Comment}:
\textit{In this paper, the authors consider the classifier learnin)g problem. To avoid the PSD cone constraint which is computationally expensive, the authors relax the problem by using linear constraints following from the Gershgorin disc perfect alignment theory, and propose an algorithm without projection onto the PSD cone.}

\textit{In this paper, the authors aim to develop an efficient algorithm for classifier learning.}

\vspace{0.4cm}
\noindent
\textbf{Overall Response}: 
We thank the reviewer for a thorough examination of our submitted manuscript. 


% %----------------------------------------------------- Q1
\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
\textit{This paper is not well-written, and the paper structure is to be improved. In Introduction, the authors should leave more space for discussing the background and motivation of the problem considered, instead of introducing the Gershgorin circle theorem. More details on the design of the algorithm should be included in Section 5.}

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
We first note that the reviewer's criticism on the writeup of the paper is in direct contradiction with comments by \textbf{reviewer EGbx}, who stated that "the paper is easy to follow" and the contribution "is clear".
Gershgorin circle theorem (GCT) and its recent extension Gershgorin disc perfect alignment (GDPA) are essential linear algebraic concepts in establishing "tightest possible" linear constraints that replace the PSD cone constraint in an SDP formulation, and thus the discussion does serve as the background and motivation of the problem considered. 
The reviewer did not specify what details of the algorithm design should be included in Section 5. 

% We thank the reviewer for this comment, and we apologize for the imprecise specification in our previous Algorithm 1.
% In the revised manuscript, we included a new metric matrix initialization procedure in Section 4.2.1, which outputs a generalized graph Laplacian matrix $\M^0$ corresponding to a balanced signed \textit{tree graph} $\cG$ and corresponding blue and red node sets $\cN_b$ and $\cN_r$. 
% These are the inputs to the pseudo-code of Algorithm 1. 
% Note also that we have rewritten the pseudo-code of Algorithm 1 in the revised manuscript for improved clarity.

% %----------------------------------------------------- Q2
\vspace{1.0cm}
\noindent
\textbf{Comment 2}: 
\textit{The contributions seem not enough for the paper to be accepted in NeurIPS. More specifically, the main contributions of this paper focus on the algorithm. Starting with the non-convex problem in Eq. (6), the authors first proposed a convex relaxation problem in Eq. (8), then reformulated the dual problem of (8) and obtained the problem (20). The authors continued to change the problem by replacing the PSD cone constraint in (20) with linear constraints. However, the authors do not provide theoretical analysis to guarantee that the final solution obtained can approximate the solution of the original problem well.}

\vspace{0.4cm}
\noindent
\textbf{Response 2}: 
The approximability of SDP relaxation to quadratically constrained quadratic programms (QCQP)---of which our semi-supervised graph classifier learning problem is a special case---is well established in the optimization literature \cite{5447068}.
We do not see a need to re-hash SDP's well-accepted bounded approximability that are already described in details in published textbooks \cite{gartner12}.
Instead, we focus on the main shortcoming of SDP relaxation---the computation complexity due to the PSD cone constraint inherent in any SDP formulation. 
To the best of our knowledge, we are the first to successfully replace the PSD cone constraint in an SDP formulation with a set of "tightest possible" linear constraints per iteration, resulting in dramatic speedup in the optimization algorithm (up to $346\times$ for large datasets). 
Further, as pointed out by \textbf{reviewer EGbx}, our proposed algorithm also serves as a template for other SDP problems, where similar algorithms that replace the PSD cone constraint with linear constraints can be designed. 
Give the broad acceptance of SDP in the optimization community \cite{doi:10.1137/1038003}, we believe that our contribution is impactful and far-reaching. 

% $b$ in L116 was set to 200 as mentioned in L246 in Section 6.1.
% %\red{Clarify pseudo-code.}
% We apologize for the unclear specification in previous Algorithm 1.
% In the rewritten Algorithm 1 in the revised manuscript, we have removed wordings ``Do 3--8" and replaced them with while loops for improved clarity.

% %----------------------------------------------------- Q3
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 3}: 
% \textit{Section 5.1. You need to provide a bound on the number of iteration of your GDPA linearization process. How many steps are required to achieve an approximate solution? Please elaborate if there is any bound on the rate of convergence.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 3}: 
% We thank the reviewer for this comment. 
% In the revised manuscript, we have added experimental comparisons with the conference version of this work that considered only graph metric matrices corresponding to positive graphs only. 
% As shown in Tables\;3 and 4 of the revised manuscript, we can see that considering graph metric matrices of more general balanced signed graphs (SGML) outperformed positive graphs (PGML) for almost all objectives $Q(\M)$ and datasets. 
% This demonstrates that it is worth the extra effort to consider the more general case of signed graphs as proposed in this paper. 

% %\blue{Cheng: We added our previous work that is also based on GDPA but within a positive graph metric space, namely, PGML \cite{yang20}. In our revised manuscript, we added the results of PGML on the objective values in Tables 3 and 4, and the classification accuracy in Tables 6 and 7. For objective values in Tables 3 and 4, our previous PGML achieved larger (for MCML, LSML, LMNN and GLR minimization problems) and smaller (for DEML maximization problem) averaged objective values over a high-complexity optimal scheme PD-cone, \textit{i.e.}, the further objective values compared to PD-cone, compared to our proposed SGML optimization scheme. As shown in the last column of Tables 3 and 4, our proposed SGML performed generally better than our previous work PGML \cite{yang20} that has generally much more restrictive metric space and has sub-optimal solutions for MCML, DEML, LSML, LMNN and GLR objectives. For classification accuracy, our previous PGML achieved comparable classification accuracy against PD-cone, and HBNB and our proposed SGML given the fact that PGML has much less time-complexity compared to the optimal scheme PD-cone. }

% %----------------------------------------------------- Q4
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 4}: 
% \textit{The abstract is very hard to follow. I would highly recommend that the authors make an attempt to rewrite it. For example, the problem studied is not clear and in L4 is stated that it is NP-hard. Complexity is high (L8) can be more precise. Last but not least, please do not state in the abstract step-by-step how you approach the problem but only state the key insights, i.e., use of GDPA theory and LPs. Removing the part, "Specifically,... per iteration" would remove a lot of unnecessary details.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 4}: 

% %----------------------------------------------------- Q5
% \vspace{1.0cm}
% \noindent
% \textbf{Comment 5}: 
% \textit{Please define the optimization problem in introduction more precisely. For example, what is optimized exactly? Please do not assume the reader is familiar with the problem under study.}

% \vspace{0.4cm}
% \noindent
% \textbf{Response 5}: 

==> reviewer_a4qs.tex <==
\textbf{Overall Comment}:
\textit{The authors propose a projection-free algorithm for the graph-based binary classifier learning problem. The main novelty is the replacement of the PSD cone constraint projection step (full eigen-decomposition) with an iterative process that requires solving linear programs. The linear constraints are derived via a Gershgorin disc perfect alignment results in combination with the smallest non-zero eigenvalue/eigenvector pair of a Laplacian matrix.}

\textit{It is not clear if the proposed method is more efficient than full eigen-decomposition. More precisely, computing the smallest eigenvalue/eigenvector pair is as hard as computing the full eigen-decomposition. The authors should handle the points below if they claim otherwise.}

\vspace{0.4cm}
\noindent
\textbf{Overall Response}: 
With due respect to the reviewer, the reviewer is factually incorrect in claiming that the computing a single extreme eigen-pair is as complex as computing full eigen-decomposition.
In the numerical linear algebra literature, there exist many fast extreme eigen-pair computation algorithms such as the power iteration \cite{MisesPraktischeVD}, Lanczos algorithm \cite{Lanczos1950AnIM} and LOBPCG \cite{Knyazev01}. 
In particular, we employ a state-of-the-art algorithm LOBPCG in our paper, with complexity $\cO(ab)$, which is clearly described in line 118 in page 3 of our submission. 
For a sparse Laplacian matrix $\cL^t$, the complexity of LOBPCG to compute a single extreme eigen-pair translates to linear time $\cO(n)$ \cite{doi:10.1137/060661624}. 
We humbly ask the reviewer to consult relevant papers on fast extreme eigen-pair computation algorithms \cite{MisesPraktischeVD,Lanczos1950AnIM,Knyazev01,doi:10.1137/060661624}, or contemporary numerical linear algebra textbooks such as \cite{vanderbei21}. 

We note further that in our extensive experiments, we have thoroughly demonstrated that by replacing the PSD cone projection with linear constraints via GDPA linearization per iteration---thus replacing full matrix eigen-decomposition with computation of a single extreme eigen-pair---we achieved up to $346\times$ speedup over competing methods. 
This dramatic speedup of replacing PSD cone projection per iteration with linear constraints thanks to GDPA linearization is also observed in the original GDPA paper \cite{yang2020signed} in the context of metric learning to speed up Frank-Wolfe iterations.
Please see \cite{yang2020signed} for details.

% %----------------------------------------------------- Q1
\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
\textit{You should provide explicit bounds on the time complexity of full eigen-solvers $\mathcal{O}(n^3)$ versus your approach, i.e., solving a sequence of LPs. What is the time complexity of your proposed approach?}

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
We first note that the reviewer is confused when requesting to compare full eigen-solvers with complexity $\cO(n^3)$ with "a sequence of LPs"; one full matrix eigen-decomposition only completes one PSD cone projection in an iterative descent algorithm such as proximal gradient (PG) \cite{Parikh31} or ADMM \cite{boyd11,8571259,cdcs_2020} that solves the SDP primal problem. 
Thus, a fair comparison is to compare the complexity of a single descent iteration, \ie, full matrix eigen-decomposition versus our proposed one extreme eigen-pair computation plus one LP.

Complexity of computing a single eigen-pair using LOBPCG is $\cO(ab)$ (described in line 118 in page 3), where $a$ is the number of entries in matrix $\cL^t$, and $b$ is the number of iterations used in LOBPCG. 
Given that Laplacian $\cL^t$ is sparse by construction, $a$ is $\cO(n)$, and $b$ is a user-determined parameter independent of $n$. 
Thus, the complexity of LOBPCG is linear \ie, $\cO(n)$, as commonly accepted in the literature \cite{doi:10.1137/060661624}. 
While the complexity of solving a LP in the classical big-O notation is still an open problem in the optimization literature \cite{vanderbei21}, it is commonly observed and accepted that an LP can be computed very efficiently using a state-of-the-art LP solver.
For example, while the worst-case running time of the popular Simplex algorithm \cite{co1998} is exponential time, in practice it has been shown to run very efficiently.
An alternative LP solver is interior point method \cite{co2009}, which may offer a faster execution time depending on the LP problem setup.
Thus, we can conclude that the complexity of one iteration of our proposed optimization strategy is  $\cO(n)$ plus one LP, while full matrix eigen-decomposition is $\cO(n^3)$. 

% We thank the reviewer for this comment, and we apologize for the imprecise specification in our previous Algorithm 1.
% In the revised manuscript, we included a new metric matrix initialization procedure in Section 4.2.1, which outputs a generalized graph Laplacian matrix $\M^0$ corresponding to a balanced signed \textit{tree graph} $\cG$ and corresponding blue and red node sets $\cN_b$ and $\cN_r$. 
% These are the inputs to the pseudo-code of Algorithm 1. 
% Note also that we have rewritten the pseudo-code of Algorithm 1 in the revised manuscript for improved clarity.

% %----------------------------------------------------- Q2
\vspace{1.0cm}
\noindent
\textbf{Comment 2}: 
\textit{What is the time complexity of computing the eigenvector corresponding to the smallest eigenvalue? Can you bound $b$ in L116? As far as I know, computing the smallest eigenvalue/vector is as hard as computing the full eigen-decomposition. Please clarify and be precise in your statements otherwise.}

\vspace{0.4cm}
\noindent
\textbf{Response 2}:
Again, the reviewer is factually incorrect in claiming that computing a single extreme eigen-pair of a matrix is as complex as computing full eigen-decomposition. 
There exist many fast eigen-pair computation algorithms in the numerical linear algebra in the literature, including power iteration method \cite{MisesPraktischeVD}, Lanczos algorithm \cite{Lanczos1950AnIM}, LOBPCG \cite{Knyazev01}, etc. 
For a sparse matrix $\cL^t$, it is commonly accepted in the numerical linear algebra literature \cite{doi:10.1137/060661624} that the complexity of LOBPCG to compute a single extreme eigen-pair is linear $\cO(n)$. 
We humbly ask the reviewer to examine related reference papers here \cite{MisesPraktischeVD,Lanczos1950AnIM,Knyazev01,doi:10.1137/060661624}, and/or recent numerical linear algebra textbooks such as \cite{vanderbei21}. 
% $b$ in L116 was set to 200 as mentioned in L246 in Section 6.1.
% %\red{Clarify pseudo-code.}
% We apologize for the unclear specification in previous Algorithm 1.
% In the rewritten Algorithm 1 in the revised manuscript, we have removed wordings ``Do 3--8" and replaced them with while loops for improved clarity.

% %----------------------------------------------------- Q3
\vspace{1.0cm}
\noindent
\textbf{Comment 3}: 
\textit{Section 5.1. You need to provide a bound on the number of iteration of your GDPA linearization process. How many steps are required to achieve an approximate solution? Please elaborate if there is any bound on the rate of convergence.}

\vspace{0.4cm}
\noindent
\textbf{Response 3}: 
Similar to popular first-order optimization methods like \textit{proximal gradient} (PG) \cite{Parikh31}, \textit{Frank-Wolfe} (FW) \cite{pmlr-v28-jaggi13} and \textit{alternating direction method of multipliers} (ADMM) \cite{boyd11,8571259,cdcs_2020}, each iteration of a descent algorithm makes progress towards an optimal solution, and the actual number of iterations executed depends entirely on the specified condition of convergence, which is pre-determined by the user. 
Hence, like PG, FW and ADMM, it is not conventional in the convex optimization literature to specify the number of iterations executed until an approximate solution is achieved.
The rate of convergence of the above first-order descent methods are all $\cO(1/t)$, which is the fastest rate of convergence possible by first-order methods \cite{doi:10.1137/1.9781611974997}. 


% We thank the reviewer for this comment. 
% In the revised manuscript, we have added experimental comparisons with the conference version of this work that considered only graph metric matrices corresponding to positive graphs only. 
% As shown in Tables\;3 and 4 of the revised manuscript, we can see that considering graph metric matrices of more general balanced signed graphs (SGML) outperformed positive graphs (PGML) for almost all objectives $Q(\M)$ and datasets. 
% This demonstrates that it is worth the extra effort to consider the more general case of signed graphs as proposed in this paper. 

% %\blue{Cheng: We added our previous work that is also based on GDPA but within a positive graph metric space, namely, PGML \cite{yang20}. In our revised manuscript, we added the results of PGML on the objective values in Tables 3 and 4, and the classification accuracy in Tables 6 and 7. For objective values in Tables 3 and 4, our previous PGML achieved larger (for MCML, LSML, LMNN and GLR minimization problems) and smaller (for DEML maximization problem) averaged objective values over a high-complexity optimal scheme PD-cone, \textit{i.e.}, the further objective values compared to PD-cone, compared to our proposed SGML optimization scheme. As shown in the last column of Tables 3 and 4, our proposed SGML performed generally better than our previous work PGML \cite{yang20} that has generally much more restrictive metric space and has sub-optimal solutions for MCML, DEML, LSML, LMNN and GLR objectives. For classification accuracy, our previous PGML achieved comparable classification accuracy against PD-cone, and HBNB and our proposed SGML given the fact that PGML has much less time-complexity compared to the optimal scheme PD-cone. }

% %----------------------------------------------------- Q4
\vspace{1.0cm}
\noindent
\textbf{Comment 4}: 
\textit{The abstract is very hard to follow. I would highly recommend that the authors make an attempt to rewrite it. For example, the problem studied is not clear and in L4 is stated that it is NP-hard. Complexity is high (L8) can be more precise. Last but not least, please do not state in the abstract step-by-step how you approach the problem but only state the key insights, i.e., use of GDPA theory and LPs. Removing the part, "Specifically,... per iteration" would remove a lot of unnecessary details.}

\vspace{0.4cm}
\noindent
\textbf{Response 4}: 
We note that the reviewer's comment on the unclear writeup is in direct contradiction with comments by reviewer EGbx, who stated that our paper "is easy to follow" and our contribution "is clear". 
The three sentences following "Specifically" describe the main technical contribution of our proposed optimization strategy, and thus we do not consider them "unnecessary details". 


% %----------------------------------------------------- Q5
\vspace{1.0cm}
\noindent
\textbf{Comment 5}: 
\textit{Please define the optimization problem in introduction more precisely. For example, what is optimized exactly? Please do not assume the reader is familiar with the problem under study.}

\vspace{0.4cm}
\noindent
\textbf{Response 5}: 
The proposed optimization strategy is clearly described in the last paragraph in the Introduction starting at line 56 of page 2 of the submission.
Again, we note that the reviewer's comment on the unclear writeup is in direct contradiction with comments by reviewer EGbx, who stated that our paper "is easy to follow" and our contribution "is clear". 

==> reviewer_a4qs_round2.tex <==
\vspace{3.0cm}
\noindent
\textbf{\Large Round 2 (13 Sept 2021)}

\noindent{\large{\textbf{Responses to Reviewer EGbx (6: Marginally aobve the acceptance threshold):}}}

%\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
Thank you for including the new comparison. My evaluation of the paper remains. Also, please note that all the other three reviewers had trouble with the paper writing and organization. The fact that I found it easy to follow (maybe due to more familiarity with the subject) does not invalidate their concerns.

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
We thank the reviewer for the updated comment.
Since the reviewer has shown diligence and interest in examining other reviews for this paper, we note that \textbf{Reviewer a4qs} has uploaded new comments on Sept 10, to which we have provided detailed responses on Sept 13. 
%We humbly ask the reviewer to consider also the new exchange in his/her evaluation.
We appreciate the reviewer's time and effort in fairly evaluating our submission based on his/her familiarity with the subject.


\vspace{1.5cm}
\noindent{\large{\textbf{Responses to Reviewer 4zJS (score increased from 5 to 6: Marginally above the acceptance threshold):}}}

%\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
I have read the other reviews and authors' responses. As I noted in my original review, I do think the paper could be interesting as a demonstration of GDPA to alleviate the numerical problem of projection onto the PSD cone. But I must also note that I am not blown away by the specific application. I thought there are issues with the technical presentation (but not the correctness of the statements). Since I see that the authors have taken steps to make some changes in this direction, I'm increasing my score from 5 to 6 (marginally above the threshold instead of below).

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
We thank the reviewer for his/her score adjustment based on our responses. 
While we are unable to convince the reviewer the targeted application (binary graph classifier) is interesting---this is a highly subjective matter---we stress that there is a sizable community in graph-based machine learning interested in the problem (as described in the paper's Introduction). 
Moreover, we believe that GDPA linearization can be more broadly applied to other SDP problems, and the targeted graph classifier in this paper serves as a useful template on how this transformation from PSD cone constraint to linear constraints can be accomplished. 


\vspace{1.5cm}
\noindent{\large{\textbf{Responses to Reviewer a4qs (score increased from 3 to 4: Ok but not good enough - rejection):}}}

\textbf{Overall Response}:
We are very grateful for the reviewer's time and effort in reading our responses carefully and providing further comments.
Please kindly see our responses to the new comments below.


\vspace{1.0cm}
\noindent
\textbf{Comment 1}: 
\textit{Note my comment was about the smallest eigenvalue/eigenvector pair. Of course, the largest eigenpair is a different discussion and Power method is a provable efficient method.}

\vspace{0.4cm}
\noindent
\textbf{Response 1}: 
The smallest eigenvalue / eigenvector pair $(\lambda, \mathbf{v})$ of a real symmetric matrix $\mathbf{M}$ is the largest eigenvalue / eigenvector pair $(-\lambda, \mathbf{v})$ of matrix $-\mathbf{M}$. 
Thus, an eigen-pair computation method such as LOBPCG that can compute the smallest eigen-pair can also compute the largest eigen-pair, and vice versa.
This is why in the numerical linear algebra literature, these are called ``extreme eigen-pair'' computation algorithms rather than ``smallest / largest eigen-pair'' computation algorithms.
With due respect to the reviewer, it is not a ``different discussion''.

Power method computes the eigen-pair corresponding to the largest MAGNITUDE eigenvalue. 
(See Section 8.2 of the classical textbook \textit{Matrix Computations} \cite{golub12} for details.)
Thus, if the smallest eigen-pair $(\lambda_{\min}, \mathbf{v})$ of a matrix $\M$ has the largest eigenvalue magnitude, i.e., $|\lambda_{\min}| \geq |\lambda_i|, \forall i$, then indeed the Power method can be used. 
Note further that even for a PSD matrix $\mathbf{M}$ where $\lambda_{\min} \geq 0$, to compute extreme eigen-pair $(\lambda_{\min}, \mathbf{v})$, one can first left-shift the spectrum by computing a \textit{linear matrix pencil} $\mathbf{M}' = \mathbf{M} - \delta \mathbf{I}$, where $\delta$ is a known shift parameter and $\mathbf{I}$ is the identity matrix, so that the largest magnitude eigenvalue $\lambda_{\min}' = \lambda_{\min} - \delta$ of $\mathbf{M}' $ corresponds to the smallest eigenvalue $\lambda_{\min} \geq 0$ of $\mathbf{M}$. 
Then one can employ Power method to compute eigen-pair $(\lambda_{\min}',\mathbf{v})$ for $\mathbf{M}'$.
(A suitable value of $\delta$ can be computed using a straightforward application of Gershgorin Circle Theorem, for example.) 
Of course, LOBPCG is one current state-of-the-art method in computing extreme eigen-pair and would be preferred over the Power method in practice.



\vspace{1.0cm}
\noindent
\textbf{Comment 2}: 
\textit{On the other hand, you need to provide a reference that proves that LOBPCG converges in exact arithmetic. I looked over [3] (http://ccm.ucdenver.edu/reports/rep149.pdf) , page 12 "...There is no theory available yet to predict accurately the speed of convergence of our new algorithms...we expect convergence of norms of residuals to be asymptotically linear with the ratio..". In particular, for a given error tolerance , how many iterations are required by LOBPCG? Does it depend on the condition number of the input matrix, etc?}

\vspace{0.4cm}
\noindent
\textbf{Response 2}: 
We first stress that the key idea of our proposal is to replace the PSD cone constraint $\mathbf{M} \succeq 0$ of a targeted SDP problem (binary graph classification) with a set of ``tightest possible'' linear constraints $\lambda^-_{\min}(\mathbf{S} \bar{\mathbf{H}} \mathbf{S}^{-1}) \geq 0$ per iteration, where $\mathbf{S} = \text{diag}(\mathbf{v})$ and $\mathbf{v}$ is the first eigenvector of the previous solution $\bar{\mathbf{H}}^{t}$. 
Our choice of LOBPCG as the extreme eigen-pair solver needs not be unique; another fast solver such as the Lanczos algorithm \cite{Lanczos1950AnIM} would also be effective.
The resulting complexity reduction---from computing a full matrix eigen-decomposition (all eigen-pairs) to computing one LP plus one extreme eigen-pair per iteration---is indisputable. 
(An entire Chapter 10 in \textit{Matrix Computation} \cite{golub12} is devoted to large sparse eigenvalue problems, where fast extreme eigen-pair methods like Lanczos are discussed.)

We are confused what the reviewer means by ``exact arithmetic''; all extreme eigen-pair algorithms in the numerical linear algebra field, including Power method, Lanczos and LOBPCG, provide approximate solutions.
See again Chapter 10 in \textit{Matrix Computation} \cite{golub12}, for example. 
Regarding convergence of LOBPCG, we first note that fast  implementation of LOBPCG is still an active area of research, where convergence issues are continuously being addressed and improved (e.g., see Section 4.3 in \cite{duersch18}). 
Linear convergence of LOBPCG is theoretically guaranteed and practically observed in later references \cite{KNYAZEV200395} than \cite{Knyazev01}; specifically, LOBPCG has complexity $\cO(n q^2)$, where $q$ defined in (5.1) of \cite{Knyazev01} quantifies the condition of the matrix $\mathbf{A}$. 
To be discussed in our response 3, this quantity is bounded in our problem and not a function of $n$.
Thus, complexity of LOBPCG is indeed $\mathcal{O}(n)$, as mentioned in our previous response.
Finally, we note that LOBPCG is computed repeatedly in our GDPA linearization algorithm, and thus LOBPCG can further benefit from warm start in subsequent computations, using previously computed eigenvectors as initial guesses. 


%\blue{The 'asymptotically linear convergence rate' mentioned in \cite{Knyazev01} (as highlighted by the reviewer) is backed up with results sho\cite{KNYAZEV200395}.wn in, \textit{e.g.}, Fig. 7.1 and Fig. 7.2 in \cite{Knyazev01}, where the green line corresponds to the exact 'asymptotically linear convergence rate' and the red lines corresponds to LOBPCG.}

%\blue{A later reference \cite{KNYAZEV200395} derives a short and sharp  convergence rate estimate for basic preconditioned eigensolvers which compute the smallest eigenvalue together with the corresponding eigenvector of a symmetric positive definite matrix, which is to stimulate a search for a more straightforward convergence proof technique that could be helpful to investigate LOBPCG.}

%\blue{\cite{KNYAZEV200395} also states that: "While an apparently sharp asymptotic convergence rate estimate for the preconditioned steepest descent method appeared in the very first paper \cite{sam58}, a sharp non-asymptotic convergence rate estimate is not yet known despite major efforts over thedecades; see \cite{ak99} for the review and references."}

%\blue{An even later reference \cite{Knyazev2017RecentIA} states that: one of the main points on LOBPCG is that, "Linear convergence is theoretically guaranteed and practically observed, since local optimality implies that LOBPCG converges at least as fast as the gradient descent. In numerical tests, LOBPCG typically shows no super-linear convergence."}


\vspace{1.0cm}
\noindent
\textbf{Comment 3}: 
\textit{In addition, scipy's implementation notes state that there are two factors that the convergence speed of LOBPCG depends on. Are these factors satisfied in your case?}

\vspace{0.4cm}
\noindent
\textbf{Response 3}: The two conditions that the reviewer is referring to are:
\begin{enumerate}
\item How well relatively separated the seeking eigenvalues are from the rest of the eigenvalues.
\item How well conditioned the problem is. This can be changed by using proper preconditioning.
\end{enumerate}
Regarding condition 1, to the best of our knowledge, the rate of convergence of all extreme eigen-pair algorithms (including Power method and Lanczos) is affected by the ``eigen-gap'' between the sought eigenvalues and the remaining eigenvalues.
In our case, our matrix $\bar{\mathbf{H}}$ in (20) is essentially the graph Laplacian matrix $\mathbf{L}$ for the positive similarity graph $\mathcal{G}$ plus two extra nodes. 
The second eigenvalue $\lambda_2$ of $\mathbf{L}$, called the \textit{Fiedler number} \cite{Chung:1997}, quantifies how ``connected'' the graph $\mathcal{G}$ is.
The initial $N$-node graph $\mathcal{G}$, specified by $\mathbf{L}$, is strongly connected by construction for binary classification. 
For the augmented graph $\bar{\mathcal{G}}$ (Fig.\;2(d)), given that dual variables $y_i$'s (acting as self-loops) do not affect graph connectivity and assuming that the two added nodes $N+1$ and $N+2$ are strongly connected to the first $N$ nodes (i.e., dual variables $z_i$'s have magnitudes $|z_i| \gg 0$ as is the typical case), the augmented graph $\bar{\mathcal{G}}$ is also strongly connected. 
Thus, $\lambda_2 \gg \lambda_1$, and this condition is easily satisfied.

Regarding condition 2, the `P' in LOBPCG stands for ``preconditioning'', which refers to the selection of a matrix $\mathbf{C}$ to improve the conditioning of the eigenvalue problem $\mathbf{A} \mathbf{x} = \lambda \mathbf{x}$ to $\mathbf{A} \mathbf{C}^{-1} \mathbf{y} = \lambda \mathbf{C}^{-1} \mathbf{y}$ (See Section 13.3 of \cite{Arbenz2016LectureNO}).
While it is unclear which particular preconditioning matrix $\mathbf{C}$ is chosen in scipy's implementation, \cite{Arbenz2016LectureNO} shows that an appropriate choice of $\mathbf{C}$ (e.g., choose $\mathbf{C}$ s.t. $\mathbf{C}^{\top} \mathbf{C} \approx \mathbf{A}$, computed using incomplete Cholesky decomposition), can significantly improve condition of the problem.
In our chosen implementation of LOBPCG (Algorithm 5.1 in \cite{Knyazev01}), we did not observe a conditioning problem.


\vspace{1.0cm}
\noindent
\textbf{Comment 4}: 
\textit{I agree with you that in practice LOBPCG could be very effective but in my opinion, such a reference is necessary to make your comparison with the direct methods .}

\vspace{0.4cm}
\noindent
\textbf{Response 4}: 
Please refer to our responses to comment 2 and 3 above.


\vspace{1.0cm}
\noindent
\textbf{Comment 5}: 
\textit{On the experimental result, I think you are right. I think I was not fair with you on that one and I will adjust my score accordingly. One comment about the experimental result that will make your submission stronger is to discuss why you consider the low error regime case, i.e., error ~ $10^4$. This is closely related to the minimum eigenvalue discussion above.}

\vspace{0.4cm}
\noindent
\textbf{Response 5}: 
We believe that the reviewer is referring to our convergence threshold $10^{-4}$ set for LOBPCG.
%\red{Cheng: why did u pick this setting? to be consistent with existing literature?}
The convergence threshold was set to $10^{-4}$ for an appropriate trade-off between the precision of the eigen-pair estimation and runtime.
We note that this threshold is consistent with existing LOBPCG literature; e.g., same convergence threshold was used in \cite{duersch18}.

\vspace{1.0cm}
\noindent
\textbf{Comment 6}: 
\textit{I still think that you need to analyze the complexity of the LP solver here. What is the complexity of "plus one LP" here? You need to specify the complexity of your selected method here. Again, in practice these worst-case bounds are pessimistic but you should discuss about it in the text and show the practical improvements in the experimental section.}

\vspace{0.4cm}
\noindent
\textbf{Response 6}: 
As discussed in our previous response, the task of designing an algorithm to solve a general LP with low complexity in the classical big-O notation is still an active research area in optimization, and is outside the scope of this paper.
Specifying the complexity of one chosen LP algorithm would mean tying the complexity of our proposal to one particular LP algorithm, which is misleading.
For example, one representative work in 2020 \cite{jiang2020faster} has complexity $\mathcal{O}(n^{2 + \max\{\frac{1}{18}, \omega-2, \frac{1-\alpha}{2}\}})$, where $\omega$ and $\alpha$ are the fast matrix multiplication exponent and its dual. 
Under the common belief that $\omega \approx 2$ and $\alpha \approx 1$, the complexity is $\mathcal{O}(n^{2.055})$, improving from previous $\mathcal{O}(n^{2.16})$ in 2019 \cite{cohen2020solving}.
Upon the reviewer's suggestion, while we can state that ``at the time of publication, the lowest complexity of a general LP solver is $\mathcal{O}(n^{2.055})$'', it would also be fair to further clarify that the LP solver field is fast-evolving, and the complexity of our proposal per iteration is not tied to a specific LP solver.

In practice, however, it is commonly observed that an appropriately chosen off-the-shelf LP solver runs significantly faster than the worst case expressed in big-O notation \cite{10.1145/3357713.3384309}.
In our experiments, we observed that our proposed algorithm was indeed very fast: $346\times$ faster than the next fastest method BCR for \texttt{madelon} with size $400$.


\vspace{1.0cm}
\noindent
\textbf{Comment 7}: 
\textit{Response 3 Is your rate of convergence $\mathcal{O}(1/t)$ as the methods that you mentioned? You show state that explicitly in your paper, if so.}

\vspace{0.4cm}
\noindent
\textbf{Response 7}: While we will be happy to include the rate of convergence (similar to previous iterative schemes like ADMM and proximal gradient) in our paper, with due respect to the reviewer, the key idea of our proposal is not on reducing the number of iterations, but on the complexity reduction per iteration, from a full matrix eigen-decomposition $\mathcal{O}(n^3)$ to one LP plus one extreme eigen-pair computation.
Following our conclusions from response 2 and response 6 above, the worst-case complexity of one LP plus one LOBPCG is $\mathcal{O}(n^{2.055} + n) = \mathcal{O}(n^{2.055})$. 
We stress again that in practice an off-the-shelf LP solver can run significantly faster than worst-case analysis, as is well-known in the optimization literature \cite{10.1145/3357713.3384309}, and LOBPCG benefits substantially from warm start due to repeated computation. 
